Exploring the Viability of Synthetic Query Generation for Relevance Prediction

Query-document relevance prediction is a critical problem in Information Retrieval systems. This problem has increasingly been tackled using (pretrained) transformer-based models which are finetuned using large collections of labeled data. However, in specialized domains such as e-commerce and healthcare, the viability of this approach is limited by the dearth of large in-domain data. To address this paucity, recent methods leverage these powerful models to generate high-quality task and domain-specific synthetic data. Prior work has largely explored synthetic data generation or query generation (QGen) for Question-Answering (QA) and binary (yes/no) relevance prediction, where for instance, the QGen models are given a document, and trained to generate a query relevant to that document. However in many problems, we have a more fine-grained notion of relevance than a simple yes/no label. Thus, in this work, we conduct a detailed study into how QGen approaches can be leveraged for nuanced relevance prediction. We demonstrate that -- contrary to claims from prior works -- current QGen approaches fall short of the more conventional cross-domain transfer-learning approaches. Via empirical studies spanning 3 public e-commerce benchmarks, we identify new shortcomings of existing QGen approaches -- including their inability to distinguish between different grades of relevance. To address this, we introduce label-conditioned QGen models which incorporates knowledge about the different relevance. While our experiments demonstrate that these modifications help improve performance of QGen techniques, we also find that QGen approaches struggle to capture the full nuance of the relevance label space and as a result the generated queries are not faithful to the desired relevance label.

==> relatedwork.tex <==
\subsection{Related Work}
\label{sec:relatedwork}

% \aditi{Structure the related work, maybe briefly summarizing the QGen for QA work, talking more about classification tasks, some things about how adding additional filtering techniques help but that's not our focus, how fluency, faithfullness to input text is studied but not faithfullness to the class-label, intriinsic metrics to measure faithfullness or define different kinds of faithfullness} 

% Synthetic Question Generation has come a long way from relying on simple but rigid heuristics \cite{Smith2011AutomaticFQ}  to using neural-network approaches, specifically seq-to-seq model \cite{serban-etal-2016-generating, Zhou2017NeuralQG, du-etal-2017-learning, du-cardie-2018-harvesting}, to now even leveraging large language models (LLMs) through prompting \cite{dai2022promptagator}. 
% Much of the work in this area has focussed on question generation in the context of QA systems.
% Below we describe some of the representative works in this area.

%\aditi{Will mostly condense the QA work}
% \paragraph{QGen for Factoid QA}
% \citet{Zhou2017NeuralQG} train a seq-to-seq model with attention to read an input sentence and generate a factoid question with respect to an answer which is contained in that sentence.
% In addition to the sentence input and the gold answer, they combine handcrafted lexical features with answer position information to generate the question, for which they train on the popular SQuaD \cite{rajpurkar2016squad} dataset.
% However, they investigate the generated question-sentence-answer triples using BLEU metric but do not explore its effect on improving downstream QA systems.
% \citet{du-etal-2017-learning} although do not use any handcrafted features but they also limit their evaluation of generated factoid questions using only BLEU and not on any downstream tasks, similar to \citet{Zhou2017NeuralQG}.
% \citet{du-cardie-2018-harvesting} go beyond using single sentence context (as \citet{du-etal-2017-learning} note that 30\% of SQuaD questions span answers beyond single sentence) for generating question.
% For this they use  coreference clusters via a gating mechanism and show improvement in the quality of generated questions.
% The importance of Question generation for improving downstream performance on QA was soon demonstrated by
% \citet{duan-etal-2017-question, yang-etal-2017-semi, dhingra-etal-2018-simple} on SQuaD,  TriviaQA-Web, BioASQ datasets, to name a few.


% With the advent of transformers \cite{vaswani2017attention} which showcased the power of attention to refer to specific parts of text, the QGen models have further improved  as now these models have the ability to process even longer context spanning multiple sentences.
% For instance, \citet{lopez2020transformer} use a GPT-2 \cite{radford2019language} language model to train a question-generation model using the passage context as input.
% They also train an answer-aware variant where they mark start and end of the answer span with special tokens in the context.
% However, they find the answer-aware variant to be under-performing for question generation (in terms of BLEU metric) than the answer-unaware model.
% They hypothesize that this is because  there is no explicit mechanism to inform the model on how to use the answer information.
% \citet{alberti-etal-2019-synthetic} use BERT \cite{devlin2018bert} to train a question-generation model conditioned on the context and answer.
% They further use round-trip consistency to generate high-quality questions, specifically, they first extract candidate answers from text, conditioned on that candidate answer and the context they generate a question and finally given the generated question and the context they ensure that the model produces the same answer as the original candidate answer.
% They find that pretraining on the above synthetic question-answer pairs results in an improvement on downstream SQuAD and NaturalQuestions \cite{} dataset.

% The newer text-to-text paradigm, specifically the T5 \cite{2020t5} and its multilingual variant mT5 \cite{xue-etal-2021-mt5} model, which are essentially transformer based encoder-decoder models, is especially conducive to the task of question generation, as it has been trained over several datasets/tasks (e.g. translation, textual entailment, question-answering, sentiment analysis etc) which are all converted to take input as text and generate output as text.
% \citet{unlu-menevse-etal-2022-framework} explore question-generation for Spoken QA task, where similar to \cite{2020t5} they use text context passage to extract answers over which they then train QGen models and finally a QA model.
% To the best of our knowledge, all of these models do some concatenation of the context passage and the answer to produce the question output.
% Additionally, the models have been applied primarily for factoid QA tasks (based mostly on SQuaD) where a single sentence contains short answer spans.

\paragraph{QGen for Open-Ended questions}
More recently, \citet{ko-etal-2020-inquisitive, chakrabarty-etal-2022-consistent, cao-wang-2021-controllable} propose approaches to generate more open-ended questions, whose answers often span multiple sentences and could be long-form.
\citet{cao-wang-2021-controllable} create a question-type ontology to guide the model to generate a particular type of question.
They essentially concatenate the question-type with the multi-sentence input to generate the question.
In the hope of controlling the question generation, they train it jointly with question focus prediction which uses semantic graphs.
The main goal of this work is to generate questions which are  diverse and illicit complex reasoning or curiosity \cite{ko-etal-2020-inquisitive}.
It is not evaluated on improving any downstream tasks.

\paragraph{QGen for Information Retrieval}
\citet{nogueira2019document, ma-etal-2021-zero} apply Qgen for improving passage retrieval tasks through data augmentation.
Given a passage, they train a QGen model to generate relevant questions.
\citet{ma-etal-2021-zero} additionally apply it for a zero-shot setting, where they use general-purpose question-passage pairs to train a QGen model, where given a passage the goal is to generate a question which is relevant to the passage.
They use the generated question-passage pairs as training data for their domain of interest.
Unlike the QGen works we saw for factoid QA above where the question is focussed towards having a specific answer span,  the question here can be a bit broad, \aditi{maybe better phrase this}, so the  degree of relevance of the question can be variable.


